Bounded Refinement Types

We present a notion of bounded quantification for refinement types and show how it expands the expressiveness of refinement typing by using it to develop typed combinators for: (1) relational algebra and safe database access, (2) Floyd-Hoare logic within a state transformer monad equipped with combinators for branching and looping, and (3) using the above to implement a refined IO monad that tracks capabilities and resource usage. This leap in expressiveness comes via a translation to "ghost" functions, which lets us retain the automated and decidable SMT based checking and inference that makes refinement typing effective in practice.

==> blank.tex <==
\input{overview-examples2}
% \input{overview-list}
\input{overview-implementation}


==> conclusion.tex <==
\section{Conclusion} \label{sec:concl}


==> copycode.tex <==
\begin{figure}
\begin{code}
copySpec h d = \w ->
  pset pcontents h w && pset plookup h     w &&
  pset pread h     w && pset pcreateFile d w &&
  pset pwrite d    w && pset pcreateF d    w &&
  pwrite (pcreateFP (select (caps w) d)))

copyRec recur s d = 
  do cs <- contents s
     forM_ cs $ \ p -> do
       x <- flookup s p
       when (isFile x) $ do
         y <- create d p
         s <- fread x
         write y s
       when (recur && (isDir x)) $ do
         y <- createDir d p
         copyRec recur x y
\end{code}
\caption{\label{fig:copysrc} Specification and Source of \texttt{copyRec}}
\end{figure}%$
% \begin{figure}[t]
% \begin{code}
% copyRec :: Bool -> s:FH -> d:FH ->
%            RIO<\w     -> CopySpec v s d,
%               ,\_ _ w -> CopySpec v s d> () 
% \end{code}
% \caption{\label{fig:copytype1} (Incorrect) Type for \texttt{copySrc}}
% \end{figure}
% \begin{figure}[t]
% \begin{code}
% bound Stable i = \w x y v -> 
%   i w => (EqP v w ||
%          (Alloc v w x && (CopyP v w x y 
%                          || DerivP v w x y)))
%       => i v 

% copyRec :: (Stable i) => 
%            Bool -> s:FH -> d:FH ->
%            RIO<\w     -> i w && CopySpec v s d,
%               ,\_ _ w -> i w && CopySpec v s d> () 
% \end{code}
% \caption{\label{fig:copytype2} (Correct) Type for \texttt{copySrc}}
% \end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> findcode.tex <==
\begin{figure}
\begin{code}
findSpec i f = \w ->
  i w && pset pcontents f w && pset plookup f w
eqc f g = \w ->
  select (caps w) f == select (caps w) g
  
bound Cmd q i p = \f v ->
  q f => i v => p f v
bound Next q i p = \f g v ->
  q f => p f v && g in active v && eqc f g v
      => p g v

findExec ::
  (Stable i, Cmd q i p, Next q i p)
  => f:FHandle<q>
  -> (g:FHandle -> RIO<p g, eqp> ())
  -> RIO<findSpec i f, \_ _ -> findSpec i f> () 
findExec f cmd = 
  do when (isFile f) $ cmd f
     when (isDir f) $
       do cs <- contents f
          forM_ cs $ \z ->
            do h <- flookup f z
              findExec h cmd
            
findWr d = \w -> findSpec d w && pset pwrite d w
prepend :: String -> d:FH -> RIO<findWr, True> ()
prepend s d = findExec dir (\f -> write f s)
\end{code}
\caption{\label{fig:findsrc} Specification and Source of \texttt{findExec}}
\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> intro-old.tex <==
Refinement types have since been used to verify 
properties ranging from partial correctness concerns 
like array bounds checking~\cite{pfenningxi98,LiquidPLDI08} 
security protocol validation~\cite{GordonTOPLAS2011,FournetCCS11}, 
web applications \cite{SwamyOAKLAND11}.
%
To ensure decidable checking several refinement
type systems including~\citep{pfenningxi98,LiquidICFP14}
restrict refinements to decidable, quantifier free logics.
%
While this ensures predictable checking and inference~\cite{LiquidPLDI08} 
it severely limits the language of specifications, and makes it hard to 
fashion simple higher order abstractions like @filter@ (let alone the more
complex ones like relational algebras and state transformers.)


\section{Introduction} \label{sec:intro}

Abstract Refinement Types~\citep{vazou13} present how abstraction over
refinement types increases expressiveness of refinement types
without increasing their complexity.
In this paper we repeat the same motif one level up:
we suggest \emph{bounded quantification} for abstract refinements. 
We describe how \textit{bounds}, \ie quantification over 
abstract refinements, increase expressiveness of abstract refinement types
without increasing their complexity.

%%%% 
%%%In other words, these Horn constraints enable a dependent 
%%%form of bounded quantification that is analogous to the 
%%%classical case.
%%%

Refinement types are used to verify semantic properties of programs
by decorating types with properties from a constrained language.
%
We choose to restrict the refinement language to qualifier-free predicates
drawn from a decidable logic
so that we enjoy decidable type checking from SMT 
solvers, 
but pay the cost of limited expressiveness.
%
Unlike us, dependent type systems (Coq~\citep{coq-book}, Agda~\citep{norell07}, \etc),
as well as some refinement type systems (\fstar~\citep{fstar}),
follow a different route:
they start from a highly expressive higher order logic 
that requires explicit, user provided proofs and work
towards developing tactics that discharge proof obligations to 
reduce the annotation burden and simplify programming.
%

Our work follows the opposite direction: we start by a 
decidable system with a constraint refinement language 
and aim to increase expressiveness.
%
Vanilla decidable refinement types have been proven ideal to reason about 
array bounds checking~\citep{pfenningxi98, LiquidPLDI08} and data
structure invariants~\citep{LiquidPLDI09}.
%
Abstract Refinement Types~\citep{vazou13} allow abstraction over refinement 
types and 
push expressiveness walls further, since they allow specification of, 
among others,
inductive and recursive invariants 
to, for example, verify list sorting algorithms.
%
We implemented Abstract Refinement Types in \toolname 
and presented that expressiveness is good enough:
\toolname has been used to verify 10.000 lines of
widely used \haskell libraries, including bytestring and Data.map.

We desired to be more expressive than Abstract Refinement Types.
For example, we were unable to specify and verify stateful computation 
or to express disjointness of two list arguments.
%
Consider, as an example, the following @product@ function
\begin{code}
product :: xs:[a] -> ys:[a] -> [(a, a)]
\end{code}
We want to express a precondition that @product@ is only applied on disjoint arguments.
%
The list elements are wrapped in the list type constructor, 
so there is no way the type of the one argument to directly refer
to the elements of the other argument.
%
As we shall see next, we can use two Abstract Refinements @p@ and @q@ 
to describe the elements of @xs@ and @ys@ respectively. 
%
Then, we enforce disjointness by quantifing  the type of @product@ by
an appropriately defined @Disjoint p q@ \textit{bound}, 
\ie a dictionary-like argument that is deleted during run-time, 
and appropriately constraints the abstract refinements @p@ and @q@ to 
describe elements of two disjoint lists. 
\begin{code}
product :: (Disjoint p q) => ...
\end{code}
%
The bound @Disjoint@ behaves as a local axiom at @product@'s definition site: 
disjointness can be assumed to prove safety of the definiton, 
and as a proof oblication at the @product@'s call-site:
the caller of  @product@ should prove that the two provided arguments are disjoint. 
%
Happily, we use the framework of liquid types to automatically prove bound obligations.


We present \textit{Bounded Refinement Types} that bound the 
abstract refinement variables that appear in the types 
to specific domains.
%
We preserve decidability by translating the bounds to functional arguments,
thus reducing Bounded to the decidable Abstract Refinement Types.
%
The paper's contributions are summarized as follows:
\begin{itemize}
\item Firstly, we provide an informal overview of Bounded Refinement Types (\S~\ref{sec:overview}), 
      describe how they can be used to precisely specify commonly used \haskell functions, 
      like @filter@, @compose@, and @foldr@.
\item Then, we demonstrate how typechecking remains decidable (\S~\ref{sec:check}) 
      by translating bounds to functions, thus reducing Bounded to Abstract Refinement Types. 
\item Finally, we provide two extensive case studies. 
      We used the power of bounds to verify correctness of relational algebra
      operators (\S~\ref{sec:database}) inspired by The power of Pi\citep{thepipower}. 
      Moreover, we used bounds to specify and verify stateful computations (\S~\ref{sec:state})
      as inspired by the Dijkstra Monad~\citep{dijkstramonad}.
\end{itemize}

We have implemented Boundend Refinement Types in \toolname~\citep{realworldliquid}.
%
The source code of the examples appearing in this paper can be found online\footnotemark[1].
\footnotetext[1]{\url{github.com/ucsd-progsys/liquidhaskell/tree/master/benchmarks/icfp15}}
%
For aesthetics and space, we have some times simplified the actual \toolname syntax.

\begin{comment}

Consider for example the function @checkGt@
that takes a list of integers @xs@ and an integer @y@
and if each element in @xs@ is less than @y@ it
returns unit, otherwise it crashes.

\begin{code}
  checkGt :: [Int] -> Int -> ()
  checkGt (x:xs) y | x < y = checkGt xs y
  checkGt []     _         = ()
\end{code}

We want to give @checkGt@ a type that checks
\textit{crash freedom}, \ie we should give it a 
precondition that states that each element of @xs@ is
less that @y@.
%
Note that if @checkGt@'s arguments were flipped than 
we could state the desired precondition using vanilla 
refinement types to name the first argument as @y@
and specify that each element of the list should be an 
Integer greater than @y@.
%
\begin{code}
  checkGt :: y:Int -> [{x:Int | x < y}] -> ()
\end{code}

\begin{code}
  checkGt :: (Gt p q) => [{x:Int | p x}] -> {y:Int | q y} -> ()
\end{code}


\begin{code}
  bound Gt p q = \x y -> p x => q y => x < y 
\end{code}


Consider for example the following function that 
takes as argument a list @xs@ of Integers,
an Integer @y@ and if @xs@ has exactly one element @x@
which is greater than @y@ then it returns @x@, 
otherwise @ex@ crashes. 
%
\begin{code}
    CheckGt :: [Int] -> Int -> ()
    checkGt (x:xs) y | x > y = checkGt xs y
    checkGt []     _         = ()
\end{code}
%
We want to type @checkGt@ in such a way as to 
prove crash freedom 
\ie give @checkGt@ a precondition that states that 
all the elements in the list @xs@ are greater that @y@. 






We start by establishing the first precondition:
the length of the input list should be exactly one.
Equipped with the measure~\citep{LiquidICFP14} @len@
that returns the length of a list, we specify a type alias
for lists with length equal to one
\begin{code}
    type MonoList a = {v:[a] | len v = 1}
\end{code}

With refinement types we establish the length precondition:
\begin{code}
    ex :: MonoList a -> a -> a
\end{code}

Next, we use Abstract Refinement Types~\citep{vazou13} to
enchance presicion. 
We abstract the signature of @ex@ over some refinement @p@
on Integers and state that if every elements of the argument
list satisfies @p@ then the result also satisfies @p@.
%
\begin{code}
    ex :: forall <p :: a -> Bool>.
          MonoList(a<p>) -> a -> a<p>
\end{code}
where informally, @Int<p>@ stands for @{v:Int | p v}@,
and @p@ is an \emph{uninterpreted function} in the refinement 
logic~\cite{NelsonOppen}.
% 
Thus, the signature states that for any refinement @p@ on @Int@,
the function takes as input a list of elements that satisfy @p@ 
and an integer
and returns as output an integer satisfying @p@. 


\begin{code}
    bound Gt p q = \x y -> p x => q y => x > y 
\end{code}

\begin{code}
    ex :: forall <p :: a -> Bool, q :: a -> Bool>.
          (Gt p q)
       => MonoList (Int<p>) -> Int<q> -> Int<p>
\end{code}

Our method is inspired by the method of~\citep{Filliatre98} 
but unlike related techniques~\cite{ynot,dijkstramonad} we
require no special support from the type system, and yet 
ensure \emph{decidable checking} of verification conditions
and \emph{inference} of loop invariants and pre- and
post- conditions via liquid typing.

\end{comment}



==> overview-list.tex <==
\subsection{Bounds for Data Types} \label{sec:overview:data}

Bounded refinements are also very useful in the first-order 
setting, for example, when working with data types.

\subsubsection*{Abstracting Refinements over Data}

Lets start by abstracting refinements over data
definitions~\cite{vazou13}. Consider the @List@ type
abstractly refined with @p :: a -> a -> Prop@, a binary relation
between two values of type @a@:
%
\begin{code}
    data List <p> a 
      = [] | (:) {h :: a, t :: List<p> a<p h>}
\end{code}
%
Intuitively, the definition states that each "tail" is a list of
elements that are @p@-related to the ``head'' @h@. That is, 
in a list $[x_1,\ldots,x_n]$ for each $1 \leq i < j \leq n$, we 
have $(\cc{p}\ x_i\ x_j)$.

\paragraph{Ordered Lists} To see why this abstraction is useful,
observe that we can define concrete refinements:
%
\begin{code}
    inc = \hd v -> hd <= v
\end{code}
%
and use them to specify and verify that sorting routines return 
lists in increasing order:
%
\begin{code}
   isort :: List a -> List<inc> a
   isort = foldr insert []

   insert :: a -> List<inc> a -> List<inc> a
   insert =  -- elided for brevity 
\end{code}

\paragraph{QuickSort} However, when we try to verify:
%
\begin{code}
    qsort        :: List a -> List<inc> a
    qsort []     = []
    qsort (x:xs) = qsort ls ++ x : qsort rs
      where
        ls       = [y | y <- xs, y <= x]  
        rs       = [z | z <- xs, x <  z]  
\end{code}
%
we run into a surprising problem: how can we type the \emph{append} 
function @(++)@ in a way that lets us prove that the concatenation 
above preserves order? 

\subsubsection*{Appending Lists}

Actually, even talking about order is presumes that we are interested
in a particular instantiation for the @List@ refinement. How can we
generically ensure that some abstract refinement @p@? Here's how; we 
define a bound:
%
\begin{code}
    bound Meet p q r = \x1 x2 -> 
      q x1 => r x2 => p x1 x2
\end{code}
%
that states that if two values @x1@ and @x2@ respectively satisfy 
the (unary) properties @q x1@ and @r x2@ then they satisfy the 
binary property @p x1 x2@. We can now use this to give append a 
type that preserves the abstract binary relation @r@:
%
\begin{code}
(++) :: (Meet p q r) => 
          List<p> a<q> -> List<p> a<r> -> List<p> a
[]     ++ ys = ys
(x:xs) ++ ys = x : xs ++ ys
\end{code}

\paragraph{To verify \cc{qsort}} \toolname automatically instantiates the 
refinements at the call to @(++)@ as: 
%
\begin{code}
    p |-> \hd v -> hd <= v      -- inc 
    q |-> \v -> v <= x 
    r |-> \v -> x < v 
\end{code}
%
This instantiation is permitted as upon instantiation, the bound 
yields the VC:
%
\begin{code}
    x1 <= x => x < x2 => x1 <= x2
\end{code}
%
which is easily validated by the SMT solver, thereby verifying that
the concatenation and hence @qsort@ produces increasingly ordered 
lists of type @List<inc> a@.

\subsubsection*{Reversing Lists}

As a final example, consider the tail recursive list @reverse@ function:
%
\begin{code}
reverse []          = []
reverse (x:xs)      = go x [] xs
  where
    go x acc []     = x : acc
    go x acc (y:xs) = go y (x : acc) xs
\end{code}  

As with append, we would like to assign @reverse@ a
refinement-generic type that does not bake order into the
signature. The natural specification is that if the input was a
@List<p> a@ then the output must be a @List<q> a@ where the
binary relation @q@ is the inverse of @p@.

\paragraph{We can specify inversion} via a bound:
%
\begin{code}
    bound Inverse p q = \x y -> p x y => q y x
\end{code}
%
and use it to type 
%
\begin{code}
    reverse :: (Inverse p q) 
            => List<p> a -> List<q> a
\end{code}

\paragraph{We can use \cc{reverse}} to specify and verify that @decsort@ 
returns lists sorted in decreasing order:
%
\begin{code}
    decsort :: List a -> List<dec> a
    decsort = reverse `compose` qsort
\end{code}
%
where @dec = \hd v -> hd >= v@. Verification proceeds by
by automatically instantiating @p@ and @q@ with the (valid) 
concrete refinements:
%
\begin{code}
    p |-> \hd v -> hd <= v
    q |-> \hd v -> v  <= hd
\end{code}

%% -- inferring
%% go :: x:a -> List<q> a<q x> -> List<p> a<p x>
%%    -> List<q> a
%% \end{code}



==> overview-old.tex <==
\section{Overview}\label{sec:overview}
\begin{comment}
<->append 
- complete cmp complete
<-> composition cmp A
- filter cmp Kaki
- state cmp Nik
\end{comment}

\subsection{Function Composition: Bringing Everything into Scope!}

We start the overview of Bounded Refinement Types by typing function composition.
%
@cmp@ is a function that takes an input two functions @f@ and @g@ and composes them.
%
\begin{code}
cmp f g x = f (g x)
\end{code}
%
Now assume that the function @f@ (resp. @g@) has some postcondition @p@ (resp. @q@) on its input @y@ (resp. @z@), \ie
%
\begin{code}
  f :: y:b -> c<p y> 
  g :: z:a -> b<q z>
\end{code}
%
Then, what is the postcondition of the composition @cmp f g@?
%
The function @cmp f g@ takes an input @x@ and returns a result that satisfies some 
relation @r@ on @x@. 
%
The relation @r@ is constraint by the fact that @p w@ should imply @r x@
\textit{for some} @w@ that satisfies @g@'s post condition @q x@.
%
The above constraint translates directly into a subtyping query:
\begin{code}
  {x:a, w:b<q x> |- c<p w> <: c<r x>}
\end{code}
We call such subtyping queries a \textit{constraint} that can be used to 
\textit{bound} Abstract Refinement Types, in that it constraints the relations
that can be used to instrantiate the abstract refinements @p@, @q@ and @r@.
%
With the above constraint the post constcondition of @cmp f g@
on an input @x@ reduces to @r x@.
%
All the above reasoning is summarized in the following type for @cmp@:
\begin{code}
cmp :: forall <p :: b -> c -> Bool, q :: a -> b -> Bool, r :: a -> c -> Bool>. 
       {x:a, w:b<q x> |- c<p w> <: c<r x>}
       f:(y:b -> c<p y>)
    -> g:(z:a -> b<q z>)
    ->   x:a -> c<r x>
\end{code}
%

The above type in theory \textit{cannot} be described by Abstract Refinement Types, 
without bounds, as there is no clear way to describe the final post condition. 
%
In practice \toolname gives function composition a type that, as the above type,
describes that 
the function @cmp f g@ takes an input @x@ and returns a result that satisfies 
@q w@
\textit{for some} @w@ that satisfies @g@'s post condition @q x@:
%
\begin{code}
cmp :: forall <p :: b -> c -> Bool, q :: a -> b -> Bool>. 
       f:(y:b -> c<p y>)
    -> g:(z:a -> b<q z>)
    ->  x:a -> exists [w:b<q x>]. c<q w>
\end{code}

This existential is required as the intermediate result @w = g x@ is not in scope at the 
type signature. 
%
Bounded refinement types address this issue simply:
In the constraints there is an environment thus variables with any properties can be assumed.
%

Bounded Refinement Types is a natural generalization of
Abstract Refinement Types with existentials, 
in that inside the constraint bounds any variable with specified types are brought 	\textit{into scope},
%
As we shall shortly see bounded refinement types have various applications.

\mypara{Using Bounded Types}

Next we describe how @cmp@ , 
\ie a function with Bounded Refinement Types, can be used.
%
As a trivial usage, consider a function @incr@ that increases its argument by one: 
%
\begin{code}
incr :: x:Nat -> {v:Nat | v == x + 1}
incr x = x + 1
\end{code}

If we compose @incr@ by itself we get a function that increases its argument by 2
\begin{code}
incr2 :: x:Nat -> {v:Nat | v = x + 2}
incr2 = cmp incr incr
\end{code}

At the call @cmp incr incr@ the abstract refinements @p@, @q@ and @r@ of @cmp@
are appropriately instantiated to @\x v -> v = x + 1@, @\x v -> v = x + 1@, and @\x v -> v = x + 2@.
%
Thus, the subtyping constraint reduces to proving the subtyping 
%
\begin{code}
  x:a, {w:b | w = x + 1} |- {v:c |  v = w + 1} <: {v:c | v = x + 2}
\end{code}
%
This in turn, using the standard refinement types regime, reduces to 
the logical implication
$$
  \forall x, w, v.  w = x + 1 \Rightarrow v = w + 1\Rightarrow v = x + 2
$$
%
that can be trivially proven by an SMT solver.

\mypara{Constraint Translation}
Constraints on functions can be thought of as 
\textit{axioms}.
%
For example,  the constraint of @cmp@ translates to the following logical axiom:
$$ 
\forall x w z. q x w \Rightarrow p w \Rightarrow r x z\ (1)
$$
%
We need to be able to apply the above axiom at any values inside @cmp@'s body.
%
To do so, we translate the constraint to a \textit{axiomatic function}
\ie a function argument whose application ensures application of the axiom. 
%
At our @cmp@ example, the axiomatic function is just a function argument with type
%
\begin{code}
        c:(x:a ->  w:b -> z:c -> {v:Unit | true && q x w => p w z => r x z)
\end{code}
%
Thus the type of @cmp@ translates to 
% 
\begin{code}
cmp :: forall <p :: b -> c -> Bool, q :: a -> b -> Bool, r :: a -> c -> Bool>. 
        c:(x:a ->  w:b -> z:c -> {v:Unit | true && q x w => p w z => r x z)
    -> f:(y:b -> c<p y>)
    -> g:(z:a -> b<q z>)
    -> x:a -> c<r x>
\end{code}

To transform the body of @cmp@ we crucially transform the code in ANF~\citep{}
so that all intermediate values are into scope.
%
Then, we apply the axiomatic functions (here @c@) whenever possible.
% 
Following this we translate the body of @cmp@ to the following safe code.
The transformation totally eliminated bounded refinement types.
%
\begin{code}
cmp c f g x 
  = let w = g x in 
     let r  = f x   in
     let _ = c x w r -- axiom application
     r   
\end{code}

Analogous transformation is applied when functions with bounded types are used.
As an example, at the call site of @cmp@ we need to provide the implementation of a function
that proves the axiom $(1)$. 
%
Unsurprisingly, a trivial function that always returns unit is such a function, 
as, by subtyping, the application is safe \texttt{iff} axiom $(1)$ holds. 
%
Thus, the call site of @cmp@ translates to 
\begin{code}
incr2 = cmp (\_ _ _ -> ()) incr incr
\end{code}

We note that the translated code is safe and does not contain any Bounded Refinement Types, 
thus its soundness is reduced to soundness of the target of the translation language; 
which is the language of Abstract Refinement Types.
%
The catch of the translation is that it is not clear when we should instantiate the axioms, 
equivalently, it is not clear when to apply the axiomatic functions and with what arguments.
%
Our translation follows the naive approach of applying the axiomatic functions whenever possible.
%
Of course the code can be expanded exponentially with respect of the number of variables, 
but since the result of the axiomatic function application is always unit, 
these applications are dead code, at run time, and can be optimized by the compiler. 


\subsection{Appending Constraint Lists}
The next application of Bounded Refinement Types is aspired by
the sorting routine quick sort.
%
Quick sort chooses a pivot element @x@,
then constructs and recursively sorts two lists:
the list of elements less than and greater than or equal to @x@.
%
Then appends the two sorted lists. 
%

We have used Abstract Refinement Types before to express list sortedness 
and verify quicksort. 
%
During verification we had to deal with a persisting issue:
how can we type list concatination to express that given 
(1)~a sorted list of elements less than @x@, and 
(2)~a sorted list of elements greater than or equal to @x@
it returns a sorted list. 
%
The difficulty of this issue arises from the fact that the desired type of 
list concatination, at its call site, naturally refers to the pivot @x@, 
but @x@ is not at scope at the definition of @(++)@.
%
Furthermore, in a type signature we are not allowed to \textit{refer} to 
the elements of a list, as there exists no quantification over them.
%
Before bounds in refinement types, the remedy was simple:
we added a ghost variable to @(++)@. 
%
With refinement type bounds we give @(++)@ a type that 
even being more verbose, does not require extra ghost variables. 
%

The bounded type for @(++)@ takes as input a sorted list @xs@ and a sorted list @ys@. 
%
Moreover, each element of @xs@ satisfies a predicate @p@ and 
each of the elements in @ys@ satisfies @q@.
%
The bounded constraint restricts @p@ and @q@ so that 
for every @x:a<p>@ if @v:a<q>@ then @x <= v@:
\begin{code}
 (++) :: forall <p :: a -> Prop, q :: a -> Prop>.
          Ord a => 
         {x:a<p> |- a<q> <: {v:a| x <= v}} 
         xs:SortedList (a<p>) -> ys:SortedList (a<q>) -> SortedList a
\end{code}

At the call site of @(++)@ we instantiate the abstract refinements @p := \v -> v < x@ 
and @q := \v -> v >= x@ thus the required constraint can be proved true:

\begin{code}
type SortedList a = [a]<{\x v -> v >= x}>

qsort :: (Ord a) => xs:[a] -> SortedList a
qsort []       = []
qsort (x:xs) = (qsort [y | y <- xs, y < x]) ++ (x:(qsort [z | z <- xs, z >= x])) 
\end{code}




%%%%% COMMENT \begin{comment}
%%%%% COMMENT \subsection{Translation By Example}
%%%%% COMMENT Translation by example: Function Composition
%%%%% COMMENT Two constraints 
%%%%% COMMENT \begin{itemize}
%%%%% COMMENT \item The post condition of @g@ on the appropriate input implies the precondition of @f@, and
%%%%% COMMENT \item the post condition of @f@ in the appropriate input implied the post condition @q@.
%%%%% COMMENT \end{itemize}
%%%%% COMMENT 
%%%%% COMMENT Let   @c1 = x:a<p>, w:b<qg x> |- c<qf w> <: c<q x>@
%%%%% COMMENT Let   @c2 = x:a<p> |- b<qg x> <: b<pf>@
%%%%% COMMENT 
%%%%% COMMENT \begin{code}
%%%%% COMMENT  cmp :: forall a b c <p, qf, pf, qg, q>. 
%%%%% COMMENT         {c1}{c2}
%%%%% COMMENT         f:(y:b<pf> -> c<qf y>)
%%%%% COMMENT     -> g:(z:a<p > -> b<qg z>)
%%%%% COMMENT     -> x: a<p> -> c<q x>
%%%%% COMMENT cmp f g x = f (g x)
%%%%% COMMENT \end{code}
%%%%% COMMENT 
%%%%% COMMENT \mypara{Step 0: Intermediate Representation}
%%%%% COMMENT 
%%%%% COMMENT \begin{code}
%%%%% COMMENT cmp a b c <p, qf, pf, qg, q> c1 c2 f g x = f (g x)
%%%%% COMMENT \end{code}
%%%%% COMMENT \mypara{Step 1 : Constraints to functions}
%%%%% COMMENT \begin{code}
%%%%% COMMENT  cmp :: forall <p, pf, qf, qg, q>. 
%%%%% COMMENT  c1: (x:a -> w:b -> z:c 
%%%%% COMMENT  -> {p x && qg x w => qf w z => q x z})
%%%%% COMMENT  c2: (x:a -> z:b -> {p x => qg x z => pf z})
%%%%% COMMENT         f:(y:b<pf> -> c<qf y>)
%%%%% COMMENT     -> g:(z:a<p > -> b<qg z>)
%%%%% COMMENT     -> x: a<p> -> c<q x>
%%%%% COMMENT cmp c1 c2 f g x = f (g x)                              
%%%%% COMMENT \end{code}
%%%%% COMMENT 
%%%%% COMMENT \mypara{Step 2: ANF}
%%%%% COMMENT \begin{code}
%%%%% COMMENT cmp c1 c2 f g x = 
%%%%% COMMENT   let w = g x in 
%%%%% COMMENT   let r = f w in 
%%%%% COMMENT   r                              
%%%%% COMMENT \end{code}
%%%%% COMMENT 
%%%%% COMMENT \mypara{Step 3: Using the axioms}
%%%%% COMMENT After @w@ is created, functional axiom @c1@ can be applied, 
%%%%% COMMENT thus we get that @w@ is an appropriate inputs for @f@.
%%%%% COMMENT After @r@ is created, functional axiom @c2@ can be applied, 
%%%%% COMMENT thus we get that @r@ is an appropriate result.
%%%%% COMMENT \begin{code}
%%%%% COMMENT cmp c1 c2 f g x = 
%%%%% COMMENT   let w = g x in 
%%%%% COMMENT   let _ = c1 x w -- {p x => qg x w => pf w}
%%%%% COMMENT   let r = f w in 
%%%%% COMMENT   let _ = c1 x w r -- {p x && qg x w => qf w r => q x r}
%%%%% COMMENT   r                              
%%%%% COMMENT \end{code}
%%%%% COMMENT 
%%%%% COMMENT Using constraint functions 
%%%%% COMMENT 
%%%%% COMMENT The abstract refinements will be automatically instantiated.
%%%%% COMMENT The trivial @\_ -> ()@ functions are appropriate instantiations of the functional arguments,
%%%%% COMMENT as the constraints do hold. Here
%%%%% COMMENT \begin{itemize}
%%%%% COMMENT \item $0 \leq x \Rightarrow w = x + 20 \Rightarrow 10 < w $ 
%%%%% COMMENT \item $0 \leq x \land w = x + 20 \Rightarrow z = w + 22 \Rightarrow z = 42 $ 
%%%%% COMMENT \end{itemize} 
%%%%% COMMENT 
%%%%% COMMENT \begin{code}
%%%%% COMMENT plus1 :: x:Nat -> {v:Nat | v == x + 20}
%%%%% COMMENT plus1 x = x + 20
%%%%% COMMENT 
%%%%% COMMENT plus2 :: x:{v:Nat | v > 10} -> {v:Nat | v == x + 22}
%%%%% COMMENT plus2 x = x + 22
%%%%% COMMENT 
%%%%% COMMENT plus42 :: x:Nat -> {v:Nat | v == x + 42}
%%%%% COMMENT plus42 = cmp plus2 plus1
%%%%% COMMENT \end{code}
%%%%% COMMENT 
%%%%% COMMENT \mypara{Step 0: Intermediate Representation}
%%%%% COMMENT 
%%%%% COMMENT \begin{code}
%%%%% COMMENT plus42 = cmp Int <\v -> v >= 0, \v -> v > 10, \x v -> v = x + 22, \x v -> v = x + 20, \x v -> v = x + 42> {Int, Int |- Int <: Int} {Int |- Int <: Int} plus2 plus1
%%%%% COMMENT \end{code}
%%%%% COMMENT 
%%%%% COMMENT \mypara{Step 1: Constraints as functions}
%%%%% COMMENT \begin{code}
%%%%% COMMENT plus42 = cmp Int <\v -> v >= 0, \v -> v > 10, \x v -> v = x + 22, \x v -> v = x + 20, \x v -> v = x + 42> (\_ _ _ -> ()) (\_ _ -> ()) plus2 plus1
%%%%% COMMENT \end{code}
%%%%% COMMENT \end{comment}


==> overview2.tex <==
\section{Overview}\label{sec:overview}

We start with a high level overview of bounded refinement types.
To make the paper self contained, we begin by recalling the notions
of abstract refinement types. Next, we introduce bounded refinements,
and show how they permit \emph{modular} higher-order specifications.
Finally, we describe how they are implemented via an elaboration
process that permits \emph{automatic} first-order verification.

\subsection{Preliminaries} 

\paragraph{Refinement Types} let us precisely specify subsets 
of values, by conjoining base types with logical predicates 
that constrain the values.  To ensure the decidability of 
type checking, these predicates are limited to decidable, 
quantifier-free, first-order logics, including the theory 
of linear arithmetic, uninterpreted functions, arrays, 
bit-vectors and so on. For example, we can write
%
\begin{code}
    type Pos     = {v:Int | 0 < v}
    type Neg     = {v:Int | v < 0}
    type IntGE x = {v:Int | x <= v} 
\end{code}
%
to specify subsets of @Int@ corresponding to values that are 
positive, negative or larger than some other value @x@ respectively.
We can specify contracts like pre- and post-conditions by 
suitably refining the input and output types of functions. 

\paragraph{We can specify preconditions} by refining input types.
For example, we specify that the function @assert@ should 
\emph{only} be called with @True@ via the type:
%
\begin{code}
    assert         :: TRUE -> a -> a
    assert True x  = x
    assert False _ = error "Provably Dead Code"
\end{code}
%
where the (input) refinement type @TRUE@ is the refinement 
of @Bool@ containing only the singleton @True@:
%
\begin{code}
    type TRUE = {v:Bool | Prop v}
\end{code}
%
(Intuitively, @Prop True@ defined to be valid (and @Prop False@ not) 
in the refinement logic.)

\paragraph{We can specify post-conditions} by refining output types. 
For example a primitive @Int@ comparison operator @leq@ can be 
assigned a type that says that the output is @True@ iff the 
first input is actually less than or equal to the second:
%
\begin{code}
leq :: x:Int -> y:Int -> {v:Bool|Prop v<=>x <= y}
\end{code}

\paragraph{Refinement Type Checking} proceeds by checking that at each
application, the types of the actual arguments are \emph{subtypes} 
of those of the function inputs, in the environment (or context) in 
which the call occurs. 
%
Consider the function:
%
\begin{code}
    checkGE     :: a:Int -> b:IntGE x -> Int
    checkGE a b = assert cmp b
      where
        cmp     = a `le` b
\end{code}
%
To verify the call to @assert@ we check that in the environment 
where @a:Int@, @b:IntGE x@, @cmp:Prop v <=> a <= b@ the type of the 
actual parameter @cmp@ is a subtype of @TRUE@. 
%
This subtyping check reduces establishing the validity of the 
\emph{verification condition}~(VC)
%
\begin{code}
 a <= b => (Prop cmp <=> a <= b) => v=cmp => Prop v
\end{code}
%
An SMT solver \cite{NelsonOppen} readily establishes the validity
of the above VC, thereby verifying @checkGE@.

% \subsection{Abstract Refinements}

\paragraph{First order refinements prevent modular specifications.} 
Consider the function that returns the largest element of a list:
% 
\begin{code}
    maximum        :: List Int -> Int 
    maximum [x]    = x
    maximum (x:xs) = max x (maximum xs)
      where
        max a b    = if a < b then b else a 
\end{code}
%
It is difficult to write a refinement type specification for 
@maximum@ that will let us verify that:
%
\begin{code}
    posMax :: List Pos -> Pos 
    posMax = maximum
    
    negMax :: List Neg -> Neg 
    negMax = maximum
\end{code}
%
Any suitable specification would have to enumerate the 
situations under which @maximum@ may be invoked 
breaking modularity.

\paragraph{Abstract Refinements} were introduced to 
overcome the above modularity problems \cite{vazou13}.
%
The main idea is that we can type @maximum@ by observing
that it returns \emph{one of} the elements in its input list.
Thus, if every element of the list enjoyed some refinement @p@
then the output value was also guaranteed to satisfy @p@.
%
Concretely, we can type the function as:
%
\begin{code}
maximum :: forall<p::Int->Prop>. List Int<p> -> Int<p>
\end{code}
%
where informally, @Int<p>@ stands for @{v:Int | p v}@,
and @p@ is an \emph{uninterpreted function} in the refinement 
logic~\cite{NelsonOppen}.
% 
Thus, the signature states that for any refinement @p@ of @Int@,
the function takes as input a list of elements that satisfy @p@ 
and returns as output an integer satisfying @p@. 

\paragraph{Notation} In the sequel, we will drop the explicit
quantification of abstract refinements; all free abstract 
refinements will be \emph{implicitly} quantified at the 
top-level (as with classical type parameters.)

\paragraph{Abstract Refinements Permit Decidable Verification}
Abstract refinements do not require the use of higher-order 
logics. Instead, \cite{vazou13} demonstrates how  abstractly 
refined signatures (like @maximum@) can be verified by viewing 
the abstract refinements @p@ as uninterpreted functions that 
only satisfy the axioms of congruence, namely:
%
\begin{code}
    forall x y. x = y => p x <=> p y
\end{code}
%
thereby preserving decidable checking \cite{NelsonOppen}.

\paragraph{Abstract Refinements are Automatically Instantiated} at call-sites,
via the abstract interpretation framework of Liquid Typing~\cite{vazou13}. 
Each instantiation yields fresh refinement variables on
which subtyping constraints are generated; these constraints
are solved via abstract interpretation yielding the instantiations.
%
Hence, we verify @posMax@ and @negMax@ by instantiating:
%
\begin{code}
    p |-> \ v -> 0 < v   -- at posMax
    p |-> \ v -> v < 0   -- at negMax
\end{code}

\subsection{Bounded Refinements}

Even with abstraction, refinement types hit various 
expressiveness walls. Consider the following example 
from~\cite{TerauchiPOPL13}. 
%
@find@ takes as input a predicate @p@, a continuation 
@k@ and an starting number @i@; it proceeds to compute
the smallest @Int@ (larger than @i@) that satisfies 
@p@, and calls @k@ with that value.
%
@ex1@ is a wrapper that passes in a continuation that
checks that the ``found'' value equals or exceeds @n@.

\begin{code}
    ex1 :: (Int -> Bool) -> Int -> ()
    ex1 p n = find p (checkGE n) n
    
    find p k i 
      | p i       = k i 
      | otherwise = find p k (i + 1)
\end{code}

\paragraph{Verification fails} as there is no way to specify that
@k@ is only called with arguments greater than @n@. 
%
First, the variable @n@ is not in scope at the function 
definition and so we cannot refer to it. 
%
Second, we could try to say that @k@ is invoked with values 
greater than or equal to @i@, which gets substituted with @n@
at the call-site. Alas, due to the currying order, @i@ too is 
not in scope at the point where @k@'s type is defined and so 
the type for @k@ cannot depend upon @i@.

\paragraph{Can Abstract Refinements Help?} Lets try to 
abstract over the refinement that @i@ enjoys, and 
type @find@ as:
%
\begin{code}
  (Int -> Bool) -> (Int<p> -> a) -> Int<p> -> a
\end{code}
%
which states that for any refinement @p@, the function takes 
an input @i@ which satisfies @p@ and hence that the continuation 
is also only invoked on a value which trivially enjoys @p@, namely @i@.
%
At the call-site in @ex1@ we can instantiate
\begin{equation}
\cc{p} \mapsto \lambda \cc{v} \rightarrow \cc{n} \leq \cc{v} \label{eq:inst:find}
\end{equation}
%
This instantiated refinement is satisfied by the parameter @n@, and
sufficient to verify, via function subtyping, that @checkGE n@ will
only be called with values satisfying @p@, and hence larger than @n@.

\paragraph{\cc{find} is ill-typed} as the signature requires that 
at the recursive call site, the value @i+1@ \emph{also} 
satisfy the abstract refinement @p@. While this holds 
for~(\ref{eq:inst:find}), it does not hold \emph{for all} @p@. 
Concretely, the recursive call generates the VC
%
\begin{code}
    ... => p i => p (i+1)
\end{code}
%
%\begin{equation}
%p\ i \Rightarrow p\ (i + 1) \label{eq:vc:find}
%\end{equation}
%
which is \emph{invalid} causing the checker to (soundly!) reject @find@.

\paragraph{We must Bound the Quantification} of @p@ to limit 
it to refinements that satisfy some constraint, in this case, 
that that @p@ is \emph{upward closed}. In the dependent setting,
where the refinements may refer to program values, these bounds 
are naturally expressed as constraints between refinements.
% Horn clauses over refinements.
%
For example we can define:
%
\begin{code} 
    bound UpClosed (p :: Int -> Prop) 
      = \x -> p x => p (x+1)
\end{code}
%
which states that @p@ is a refinement that is \emph{upward closed}, 
\ie satisfies @forall x. p x =>  p (x+1)@.

\paragraph{Bound Constraints are Horn Clauses} over the refinements. 
That is, they correspond to a series of implications of the 
form: $$P_1 \Rightarrow \ldots \Rightarrow P_n$$ where each $P_i$ 
is either
%
(1)~a \emph{concrete} formula from the refinement logic 
   (with arbitrary boolean connectives), or,
%
(2)~an application of an \emph{abstract} refinement 
   (with no boolean connectives).
%
This form of constraints is not arbitrary -- it corresponds 
directly to the subtyping constraints that arise in refinement
type checking~\cite{HMC}, and hence, crucially keeps checking
and inference decidable.

We can use the bound to type @find@ as:
%
\begin{code}
    find :: (UpClosed p) => (Int -> Bool) 
                         -> (Int<p> -> a) 
                         ->  Int<p> -> a
\end{code}
%
This time, the checker is able to use the bound to 
verify the VC. We do so in a way that the VCs remain 
quantifier free and hence, within the SMT solver's 
decidability borders~(\S~\ref{sec:overview:implementation}).

\paragraph{At the call to \cc{find}} inside @ex1@, we perform 
the instantiation~(\ref{eq:inst:find}) which generates the 
\emph{additional} VC generated by plugging in the concrete 
refinements in the bound constraint:
%
\begin{code}
    n <= x => n <= x + 1
\end{code}
%
The SMT solver easily checks the validity of the VC 
and hence this instantiation, thereby verifying @ex1@, 
\ie statically verifying that the assertion inside 
@checkGE@ cannot fail.
%
Crucially, we can also \emph{automatically synthesize} 
instantiations that satisfy the (Horn) constraint via 
the framework of Liquid Typing \cite{LiquidPLDI08}, 
which makes using such bounds palatable in practice.

\subsection{Bounds for Higher-Order Functions}

% @find@ is an simple example that serves to illustrate how bounds work. 

Next, we show how bounds drastically stretch the scope 
of refinement typing by allowing precise specifications 
for several canonical higher-order functions.

\subsubsection*{Function Composition}\label{sec:compose}

Our first example is the @compose@ function
%
\begin{code}
    compose f g x = f (g x)
\end{code}
%
What is a modular specification for @compose@ that lets us check @ex2@? 
%
\begin{code}
    type Plus x y = {v:Int | v = x + y}
    
    ex2    :: n:Int -> Plus n 2
    ex2    = incr `compose` incr 
    
    incr   :: n:Int -> Plus n 1
    incr n = n + 1 
\end{code}

% \paragraph{Typing \texttt{compose}} The challenge here is \emph{chaining} the dependencies 

\paragraph{The challenge is to chain the dependencies} between the
input and output of @g@ and the input and output of @f@ to 
obtain a relationship between the input and output of the 
composition. We can capture the notion of chaining in a bound:
%
\begin{code}
    bound Chain f g r = \x y z -> 
      g x y => f y z => r x z
\end{code}
%
which states that for any @x@, @y@ and @z@, if
%
(1) @x@ and @y@ are related by @g@, and
(2) @y@ and @z@ are related by @f@, then
(3) @x@ and @z@ are related by @r@.

We can use this bound to type @compose@ using three abstract 
refinements @f@, @g@ and @r@ respectively relating the inputs 
and outputs of the arguments @f@ and @g@ and their composed 
result. (Here, @c<r x>@ abbreviates @{v:c | r x v}@.)

\begin{code}
    compose :: (Chain f g r) => (y:b -> c<f y>) 
                             -> (z:a -> b<g z>) 
                             -> (x:a -> c<r x>)
\end{code}

\paragraph{To verify \cc{ex2}} we instantiate, at the call to @compose@,
%
\begin{code}
    f, g |-> \x v -> v = x + 1
       r |-> \x v -> v = x + 2
\end{code}
%
The above instantiation satisfies the bound, as shown by the validity 
of the derived substituted VC: 
%
\begin{code}
    y = x + 1 => z = y + 1 => z = x + 2
\end{code}
%
and hence, we can check that @ex2@ implements its specified type.

Previously, \cite{vazou13} describes a way to type @compose@ 
using abstract refinements and an ad-hoc form of existential 
types. Bounds let us express chaining without any extra machinery.


\subsubsection*{List Filtering}

Next, consider the List @filter@ function:
%
\begin{code}
    filter f (x:xs)
      | f x         = x : filter f xs
      | otherwise   = filter f xs
    filter _ []     = []
\end{code}
%
What type signature for @filter@ would let us check @positives@?
%
\begin{code}
    positives :: [Int] -> [Pos]
    positives = filter isPos  
      where
        isPos x = 0 < x
\end{code}
%
Such a signature would have to relate the @Bool@ returned by 
@f@ with the property of the @x@ that it checks for. 

Typed Racket's latent predicates~\cite{typedracket} 
account for this idiom, but are a special construct 
limited to @Bool@-valued ``type'' tests, and not 
arbitrary invariants.
%
Another, approach is to avoid the so-called 
``Boolean Blindness'' that accompanies 
@filter@ by instead using option types 
and @mapMaybe@.

\paragraph{We overcome blindness using a witness} bound:
%
\begin{code}
   bound Witness p w = \x b -> 
     Prop b => w x b => p x
\end{code}
%
which says that the refinement @w@ \emph{witnesses} the 
refinement @p@, meaning that for any boolean @b@ such 
that @w x b@ holds, if @b@ is @True@ then @p x@ also holds. 

\paragraph{\cc{filter} can be given a type} that says that the output values
all enjoy a refinement @p@ as long as the test predicate @f@ returns
a boolean that witnesses @p@:
%
\begin{code}
   filter :: (Witness p w) => (x:a -> Bool<w x>) 
                           -> List a 
                           -> List a<p>
\end{code}

\paragraph{To verify \cc{positives}} we infer the following type and 
instantiations for the abstract refinements @p@ and @w@ at the 
call to @filter@:
%
\begin{code}
    isPos :: x:Int -> {v:Bool | Prop v <=> 0 < v}
    p     |-> \v   -> 0 < v
    w     |-> \x b -> Prop b <=> 0 < x
\end{code}

\subsubsection*{List Folding}

Next, consider the list fold-right function:
%
\begin{code}
    foldr :: (a -> b -> b) -> b -> List a -> b
    foldr op b []     = b
    foldr op b (x:xs) = x `op` foldr op b xs
\end{code}
%
Suppose that we wish to prove that:
%
\begin{code}
    ex3 :: xs:List a -> {v:Int | v = len xs}
    ex3 = foldr (\_ -> incr) 0
\end{code}
%
where @len@ is a \emph{logical} or \emph{measure} 
function used to represent the number of elements of
the list in the refinement logic~\cite{LiquidICFP14}:
%
\begin{code}
    measure len :: List a -> Nat
    len []      = 0
    len (x:xs)  = 1 + len xs
\end{code}

\paragraph{We specify induction as a bound.} Concretely, let
(1)~@inv@ be an abstract refinement relating a list @xs@ 
    and the result @b@ obtained by folding over it, and
(2)~@step@ be an abstract refinement relating the 
    inputs @x@, @b@ and output @b'@ passed to and 
    obtained from the accumulator @op@ respectively.
%
Then
%
\begin{code}
    bound Inductive inv step = \x xs b b' -> 
      inv xs b => step x b b' => inv (x:xs) b'
\end{code}
%
states that @inv@ is closed under @step@. 

\paragraph{We can give \cc{foldr} at type} that says, that the 
function \emph{outputs} a value that is built inductively
over the entire \emph{input} list:
%
\begin{code}
    foldr :: (Inductive inv step) 
          => (x:a -> acc:b -> b<step x acc>)
          -> b<inv []>
          -> xs:List a
          -> b<inv xs>
\end{code}
%
That is, for any invariant @inv@ that is inductive 
under @step@, if the initial value @b@ is @inv@-related
to the empty list, then the folded output is @inv@-related
to the input list @xs@.

\paragraph{We verify \cc{ex3}} by inferring, at the call to @foldr@
%
\begin{code}
    inv  |-> \xs v   -> v = len xs
    step |-> \x b b' -> b' = b + 1
\end{code}
%
The SMT solver validates the VC obtained by plugging the 
above into the bound, and the final output type of the 
instantiated signature for @foldr@ yields the desired 
output type for @ex3@.

%  LocalWords:  UpClosed IntGE ok Bool listMax xs Pos Neg posMax negMax forall
%  LocalWords:  QuickSort incr mapMaybe


==> rules.tex <==
\NV{Questions on the Abstract Refinement paper:}
\NV{1. WF-Abs-alpha: why we put alpha into the environment?}
\NV{2. We do we need the first two well-formedness rules?}
\newcommand\interp[1]{\ensuremath{[\! | #1 |\!]}}


\begin{figure}[!ht]
\judgementHead{Well-Formedness}{\isWellFormed{\Gamma}{\sigma}}

$$
\inference
  {}
  {\isWellFormed{\Gamma}{\true(\vref)}}
  [\wtTrue]
$$

$$
\inference
    {\isWellFormed{\Gamma}{\areft(\vref)} && 
     \hastype{\Gamma}{\rvapp{\rvar}{e} \ \vref}{\tbbool}
    }
    {\isWellFormed{\Gamma}{(\areft \wedge \rvapp{\rvar}{e})(\vref)}}
    [\wtRVApp]
$$

$$\inference
    {\hastype{\Gamma, \vref:b}{\reft}{\tbbool} \quad 
     \isWellFormed{\Gamma, \vref:b}{\areft(\vref)}
    }
    {\isWellFormed{\Gamma}{\tpref{b}{\areft}{\reft}}}
    [\wtBase]
$$

$$
\inference
    {
	\hastype{\Gamma}{\reft}{\tbbool} &&
    \isWellFormed{\Gamma}{\tau_x} &&
	\isWellFormed{\Gamma, x:\tau_x}{\tau}
    }
    {\isWellFormed{\Gamma}{\trfun{x}{\tau_x}{\tau}{\reft}}}
    [\wtFun]
$$


$$\begin{array}{ccc}
\inference
  {\isWellFormed{\Gamma, \rvar:\tau}{\sigma}}
  {\isWellFormed{\Gamma}{\tpabs{\rvar}{\tau}{\sigma}}}
  [\wtPred]
&
\quad
&
\inference
    {\isWellFormed{\Gamma}{\sigma}}
    {\isWellFormed{\Gamma}{\ttabs{\alpha}{\sigma}}}
    [\wtPoly]
\end{array}$$

\medskip \judgementHead{Subtyping}{\isSubType{\Gamma}{\sigma_1}{\sigma_2}}

$$
\inference
   {\text{SMT-Valid}(\inter{\Gamma} \land \inter{\areft_1\ \vref} \Rightarrow \inter{\reft_1} 
                 \Rightarrow \inter{\areft_2\ \vref} \land \inter{\reft_2})}
   {\isSubType{\Gamma}{\tpref{b}{\areft_1}{\reft_1}}{\tpref{b}{\areft_2}{\reft_2}}}
   [\tsubBase]
$$

$$
\inference
   {%\text{Valid}(\inter{\Gamma}\land \inter{e_1} \Rightarrow \inter{e_2}) \\
	\isSubType{\Gamma}{\tau_2}{\tau_1} &
	\isSubType{\Gamma, x_2:{\tau_2}}{\SUBST{\tau_1'}{x_1}{x_2}}{\tau_2'}	
   }
   {\isSubType{\Gamma}
	  {\trfun{x_1}{\tau_1}{\tau_1'}{\reft_1}}
	  {\trfun{x_2}{\tau_2}{\tau_2'}{\true}}
}[\tsubFun]
$$


$$
\inference
   {\isSubType{\Gamma, \rvar:\tau}{\sigma_1}{\sigma_2}}
   {\isSubType{\Gamma}{\tpabs{\rvar}{\tau}{\sigma_1}}{\tpabs{\rvar}{\tau}{\sigma_2}}}
   [\tsubPred]
$$
$$
\inference
   {\isSubType{\Gamma}{\sigma_1}{\sigma_2}}
   {\isSubType{\Gamma}{\ttabs{\alpha}{\sigma_1}}{\ttabs{\alpha}{\sigma_2}}}
   [\tsubPoly]
$$

\medskip \judgementHead{Type Checking}{$\hastype{\Gamma}{e}{\sigma}$}

$$
\inference
  {  \hastype{\Gamma}{e}{\sigma_2} && \isSubType{\Gamma}{\sigma_2}{\sigma_1} 
  && \isWellFormed{\Gamma}{\sigma_1}
  }
  {\hastype{\Gamma}{e}{\sigma_1}}
  [\tsub]
$$

$$
\inference
  {}
  {\hastype{\Gamma}{c}{\tc{c}}}
  [\tconst]
$$

$$
\inference
  {x: \tpref{b}{\areft}{\reft} \in \Gamma}
  {\hastype{\Gamma}{x}{\tpref{b}{\areft}{e \land \vref = x}}}
  [\tbase]
$$
$$
\inference
  {x:\tau \in \Gamma}
  {\hastype{\Gamma}{x}{\tau}} 
  [\tvariable]
$$

$$
\inference
   {\hastype{\Gamma, x:\tau_x}{e}{\tau} 
    && \isWellFormed{\Gamma}{\tau_x}
   }
   {\hastype{\Gamma}{\efunt{x}{\tau_x}{e}}{\tfun{x}{\tau_x}{\tau}}}
   [\tfunction]
$$
$$
\inference
   {\hastype{\Gamma}{e_1}{\tfun{x}{\tau_x}{\tau}} 
   &&  \hastype{\Gamma}{e_2}{\tau_x}
   }
   {\hastype{\Gamma}{\eapp{e_1}{e_2}}{\SUBST{\tau}{x}{e_2}}}
   [\tapp]
$$
$$
\inference
  {\hastype{\Gamma, \alpha}{e}{\sigma}}
  {\hastype{\Gamma}{\etabs{\alpha}{e}}{\ttabs{\alpha}{\sigma}}}
  [\tgen]
\qquad
\inference
  {\hastype{\Gamma}{e}{\ttabs{\alpha}{\sigma}} && 
   \isWellFormed{\Gamma}{\tau}
  }
  {\hastype{\Gamma}{\etapp{e}{\tau}}{\SUBST{\sigma}{\alpha}{\tau}}}
  [\tinst]
$$
$$
\inference
    {\hastype{\Gamma, \rvar:\tau}{e}{\sigma} &&
     \isWellFormed{\Gamma}{\tau} 
     % \tau \mbox{ is non-refined } 
     %\isWellFormed{\Gamma}{\tpabs{p}{\tau}{\pi}} && 
     %p \notin \fv{e}
    }
    {\hastype{\Gamma}{\epabs{\rvar}{\tau}{e}}{\tpabs{\rvar}{\tau}{\sigma}}}
    [\tpgen]
$$
$$
\inference
    {\hastype{\Gamma}{e}{\tpabs{\rvar}{\tau}{\sigma}} && 
     \hastype{\Gamma}{\efunbar{x:\tau_x}{\reft'}}{\tau}
    }
    {\hastype{\Gamma}
             {\epapp{e}{\efunbar{x:\tau_x}{\reft'}}}
             {\rpinst{\sigma}{\rvar}{\efunbar{x:\tau_x}{\reft'}}}
    }
    [\tpinst]
$$
\caption{\textbf{Static Semantics: Well-formedness, Subtyping and Type Checking}}
\label{fig:rules}
\end{figure}


\begin{figure}[!ht]
\judgementHead{Well-Formedness}{\isWellFormed{\Gamma}{\sigma}}

$$
\inference{
   \isWellFormed{\Gamma}{\Gamma_\constraint}             && 
	\isWellFormed{\Gamma, \Gamma_\constraint}{r_1} &&
	\isWellFormed{\Gamma, \Gamma_\constraint}{r_2} &&
	\isWellFormed{\Gamma}{\tau}
}{
	\isWellFormed{\Gamma}{\{\isSubType{\Gamma_\constraint}{r_1}{r_2}\} \carrow  \tau}
}[\wfBounded]
$$

$$
\inference{
}{
	\isWellFormed{\Gamma}{\emptyset}
}[\wfGammaEmpty]
$$
$$
\inference{
	\isWellFormed{\Gamma_1}{\sigma} && \isWellFormed{\Gamma_1, x\colon\sigma}{\Gamma_2}
}{
	\isWellFormed{\Gamma_1}{x\colon\sigma, \Gamma_2}
}[\wfGammaNonEmpty]
$$


\medskip \judgementHead{Subtyping}{\isSubType{\Gamma}{\sigma_1}{\sigma_2}}

$$
\inference{
    \isSubType{\Gamma_\constraint}{r_1}{r_2} && 
    \isSubType{\Gamma}{\tau_1}{\tau_2}
}{
   \isSubType{\Gamma}{\{\isSubType{\Gamma_\constraint}{r_1}{r_2}\} \carrow  \tau_1}{\tau_2}
}[\tsubPoly]
$$

\medskip \judgementHead{Type Checking}{$\hastype{\Gamma}{e}{\sigma}$}
$$
\inference{
	\text{fresh}\ x &&
	\hastype{\Gamma, x\colon\tref{\tbunit}{\interp{\isSubType{\Gamma_\constraint}{r_1}{r_2}}}}{e}{\tau}
}{
  \hastype{\Gamma}{e}{\{\isSubType{\Gamma_\constraint}{r_1}{r_2}\} \carrow  \tau}
}[\tsub]
$$
$$
\inference{
  \hastype{\Gamma}{e}{\{\isSubType{\Gamma_\constraint}{r_1}{r_2}\} \carrow  \tau}
  && \isSubType{\Gamma, \Gamma_\constraint}{r_1}{r_2}
}{
  \hastype{\Gamma}{e}{\tau}
}[\tsub]
$$
\caption{\textbf{Extensions In Reality}}
\label{fig:rules}
\end{figure}


\begin{figure}[!ht]
\judgementHead{Well-Formedness}{\isWellFormed{\Gamma}{\sigma}}

$$
\inference{
	\isWellFormed{\Gamma}{\constraint} &&
	\isWellFormed{\Gamma}{\tau}
}{
	\isWellFormed{\Gamma}{\tconstraint{\constraint}{\tau}}
}[\wfBounded]
$$

\medskip \judgementHead{Subtyping}{\isSubType{\Gamma}{\sigma_1}{\sigma_2}}

$$
\inference{
    \isSubType{\Gamma_\constraint}{r_1}{r_2} && 
    \isSubType{\Gamma}{\tau_1}{\tau_2}
}{
   \isSubType{\Gamma}
                    {\tconstraint{\isSubType{\Gamma_1}{r_{11}}{r_{12}}}{\tau_1}}
                    {\tconstraint{\isSubType{\Gamma_2}{r_{21}}{r_{22}}}{\tau_2}}
}[\tsubPoly]
$$

\medskip \judgementHead{Type Checking}{$\hastype{\Gamma}{e}{\sigma}$}
$$
\inference{
	\hastype{\Gamma}{e}{\tconstraint{\isSubType{\Gamma'}{r_1}{r_2}}{\tau}} &&
	\isSubType{\Gamma, \Gamma'}{r_1}{r_2}
}{
  \hastype{\Gamma}{e\ \econstantconstraint}{\tau}
}
$$
$$
\inference{
	\text{fresh}\ x &&
	\isWellFormed{\Gamma}{\phi} && \hastype{\Gamma, x\colon\tref{\tbunit}{\inter{\constraint}}}{e}{\tau}
}{
  \hastype{\Gamma}{(\econstraint{e})}{\tconstraint{\constraint}{\tau}}
}
$$
\caption{\textbf{Extensions In Theory}}
\label{fig:rules}
\end{figure}



\begin{figure}[!ht]
\judgementHead{Well-Formedness-Constraint}{\isWellFormed{\Gamma}{\constraint}}
$$
\inference{
	\isWellFormed{\Gamma}{\Gamma'} 
	&& \isWellFormed{\Gamma, \Gamma'}{r_1}
	&& \isWellFormed{\Gamma, \Gamma'}{r_2}
}{
	\isWellFormed{\Gamma}{(\isSubType{\Gamma'}{r_1}{r_2})}
}
$$

$$
\inference{
}{
	\isWellFormed{\Gamma}{\emptyset}
}% [\wfGammaEmpty]
\qquad
\inference{
	\isWellFormed{\Gamma_1}{\sigma} && \isWellFormed{\Gamma_1, x\colon\sigma}{\Gamma_2}
}{
	\isWellFormed{\Gamma_1}{x\colon\sigma, \Gamma_2}
}% [\wfGammaNonEmpty]
$$

\caption{\textbf{More Rules}}
\label{fig:rules}
\end{figure}

\begin{figure}
$$
\begin{array}{l}
\interp{\isSubType{\Gamma}{\tpref{b}{\areft_1}{\reft_1}}{\tpref{b}{\areft_2}{\reft_2}}} \\
  \qquad =\forall(dom(\Gamma), \vref) . \inter{\Gamma} \land \inter{\areft_1\ \vref} \Rightarrow \inter{\reft_1} 
                 \Rightarrow \inter{\areft_2\ \vref} \land \inter{\reft_2} 
\end{array}
$$
\label{fig:rules}
\end{figure}


\NV{make clear how forall is an expression}

\subsection{Translation}
Let $n$ be the the maximum number of constraints that appear in a type in the program. 
Then 





$$\begin{array}{rclcrcl}
\tx{\true\ \vref} & \defeq 
  & \true  
  & \quad \quad &

\tx{\tpabs{\rvar}{\tau}{\sigma}} & \defeq 
  & \tfun{\rvar}{\tx{\tau}}{\tx{\sigma}} \\

\tx{(\areft \land \rvapp{\rvar}{e})\ \vref} & \defeq 
  & \tx{\areft\ \vref} \land \eapp{\eapp{\rvar}{\overline{e}}}{\vref} 
  & \quad \quad &

\tx{\ttabs{\alpha}{\sigma}} & \defeq 
  & \ttabs{\alpha}{\tx{\sigma}} \\

\tx{\tpref{b}{\areft}{\reft}} & \defeq 
  & \tref{b}{\reft \land \tx{\areft\ \vref}} 
  & \quad \quad &

\tx{\tfun{x}{\tau_1}{\tau_2}} & \defeq 
  & \tfun{x}{\tx{\tau_1}}{\tx{\tau_2}} 
%\tx{\trfun{x}{\tau_1}{\tau_2}{\reft}} \defeq 
%  & \trfun{x}{\tx{\tau_1}}{\tx{\tau_2}}{\tx{\reft}} \\
\end{array}$$
Similarly, we translate \corelan terms $e$ to \conlan 
terms $\tx{e}$ by converting refinement abstraction and application 
to $\lambda$-abstraction and application
$$\begin{array}{rclcrcl}
\tx{x} & \defeq & x & \quad \quad \quad & \tx{c} & \defeq & c \\
\tx{\efunt{x}{\tau}{e}} & \defeq & \efunt{x}{\tx{\tau}}{\tx{e}} & \quad & \tx{\eapp{e_1}{e_2}} & \defeq & \eapp{\tx{e_1}}{\tx{e_2}} \\
\tx{\etabs{\alpha}{e}} & \defeq & \etabs{\alpha}{\tx{e}} & \quad & \tx{\etapp{e}{\tau}} & \defeq & \eapp{\tx{e}}{\tx{\tau}} \\
\tx{\epabs{\rvar}{\tau}{e}} &\defeq & \efunt{\rvar}{\tx{\tau}}{\tx{e}} & \quad & \tx{\epapp{e_1}{e_2}} &\defeq & \eapp{\tx{e_1}}{\tx{e_2}}
\end{array}$$









==> supplemented.tex <==
\paragraph{Implementation}
We have implemented Bounded Refinement Types in \toolname.
Our code and examples can be found on github at 
\url{https://github.com/ucsd-progsys/liquidhaskell/tree/master/benchmarks/icfp15}.

\paragraph{Soundness} 
Below we prove soundness of \boundedcorelan by reduction to \corelan.

\begin{theorem*}[Semantics Preservation]
\label{theorem:operational}
If $\txexpr{\emptyset}{\emptyset}{e}{e'}$ and
   $e \boundedgoestostar{c}$ 
then $e' \goestostar{c}$.
\end{theorem*}

\begin{proof}
By assumption, there exists a sequence 
$e \equiv e_1 \boundedgoesto{e_2} \boundedgoesto{} \dots
\boundedgoesto{e_n\equiv c} $.
%
Let $i$ be the largest index in which rule \rtobound was applied.
%
Then, for some $\phi$ and $\phi'$, 
$e_i$ contains a sub-expression of the form 
$\econstantconstraint{(\econstraint{\phi}{e_i^0})}{\phi'}$.
%
Let $e_i^1$ be the expression we get if we replace 
$\econstantconstraint{(\econstraint{\phi}{e_i^0})}{\phi'}$
with $e_i^0$ in $e_i$.
%
By the way we choose $i$, there exist a sequence 
$e_i^1 \goestostar{c}$.

Let $e_i^2$
be the expression we get if we replace 
$\econstantconstraint{(\econstraint{\phi}{e_i^0})}{\phi'}$
with $\eapp{(\efunt{f}{\txbound{\phi}}{e_i^0})}{(\ctofun{\phi'})}$ in $e_i$.
%
Then, since $f$ does not appear in $e_i^0$,
$e_i^2 \goestostar{c}$.
%
Finally, 
let $g \defeq \ctofun{\phi'}$, then
by the definition of 
$\ctofun{\cdot}$
we have that  $\forall e_1 \dots e_n$ 
if 
there exists a type $\tau$ such that
$\emptyset \vdash g \ e_1 \dots e_n : \tau $,
then $g \ e_1 \dots e_n \goestostar{true}$.
%
Thus, for any expression, 
if $e \goestostar{c}$, then $\elett{t}{f \ e_1 \dots e_n}{e}\goestostar{c}$

From the above, by the way we choose $i$ we have that 
there exists a sequence 
%
$\txex{e_i} \hookrightarrow \dots \hookrightarrow {c}$.

Since $n$ is finite, we iteratively apply the above procedure to 
$e \equiv e_1\boundedgoesto{} \dots \boundedgoesto{} \txex{e_i}\hookrightarrow \dots \hookrightarrow {c}$.
until we get the sequence $ {\txex{e}}\goestostar{c}$.
\end{proof}

The soundness of \corelan as stated in~\cite{vazou13}:  

\begin{theorem*}[Soundness of \corelan]
\label{theorem:core} %\cite{vazou13}
If   $\hastype{\emptyset}{e}{\sigma}$ 
then $e \not \goestostar{\ecrash}$.
\end{theorem*}

\begin{theorem*}[Soundness]
\label{theorem:bounded}
If $\txexpr{\emptyset}{\emptyset}{e}{e'}$ and
   $\hastype{\emptyset}{e'}{\sigma}$ 
then $e \not \boundedgoestostar{\ecrash}$.
\end{theorem*}
\begin{proof}
Since $\hastype{\emptyset}{e'}{\sigma}$ then by Soundness of \corelan
$e' \not \goestostar{\ecrash}$ and thus by Semantics Preservation $e \not \boundedgoestostar{\ecrash}$. 
\end{proof}

==> typechecking.tex <==
\section{Syntax and Semantics}\label{sec:check}


Next, we present a core calculus \corelan that formalizes the notion
of abstract refinements. We start with the syntax (\S~\ref{sec:syntax}),
present the typing rules (\S~\ref{sec:typing}), show soundness 
via a reduction to contract calculi \cite{Knowles10,Greenberg11}
(\S~\ref{sec:soundness}), and inference via Liquid types (\S~\ref{sec:infer}).

\subsection{Syntax}\label{sec:syntax}

Figure~\ref{fig:syntax} summarizes the syntax of our core 
calculus \corelan which is a polymorphic $\lambda$-calculus 
extended with abstract refinements. 
%
We write 
$b$, 
$\tref{b}{\reft}$ and 
$\tpp{b}{\areft}$ 
to abbreviate 
$\tpref{b}{\true}{\true}$, 
$\tpref{b}{\true}{\reft}$, and
$\tpref{b}{\areft}{\true}$ respectively. 
We say a type or schema is \emph{non-refined} if all the 
refinements in it are $\true$. We write $\overline{z}$ 
to abbreviate a sequence $z_1 \ldots z_n$.


\mypara{Expressions}
\corelan\ expressions include the standard variables $x$, 
primitive constants $c$, $\lambda$-abstraction $\efunt{x}{\tau}{e}$,
application $\eapp{e}{e}$, type abstraction $\etabs{\alpha}{e}$,
and type application $\etapp{e}{\tau}$. The parameter $\tau$ in 
the type application is a \emph{refinement type}, as described shortly.
The two new additions to \corelan are the refinement abstraction
$\epabs{\rvar}{\tau}{e}$, which introduces a refinement variable 
$\rvar$ (together with its type $\tau$), which can appear in refinements
inside $e$, and the corresponding refinement application $\epapp{e}{e}$.
%
%where the argument, is of the form $\efun{\bar{x}{e}}$ which is
%an abbreviation for $\efun{x_1 \ldots x_n}{e}$.
%which is of the form $\ptype{\bar{\tau}}$ which is an 
%abbreviation for $\ptype{tau_1 \rightarrow \ldots \tau_n}$,
%where each $\tau_i$ is a simple (non-function) type.

\mypara{Refinements}
A \emph{concrete refinement} \reft is a boolean valued expression \reft 
drawn from a strict subset of the language of expressions which
includes only terms that 
(a)~neither diverge nor crash, and 
(b)~can be embedded into an SMT decidable refinement logic including 
the theory of linear arithmetic and uninterpreted functions.
%
An \emph{abstract refinement} \areft is a conjunction of refinement
variable applications of the form $\rvapp{\pi}{e}$.

\mypara{Types and Schemas}
The basic types of \corelan include the base types $\tbint$ and $\tbbool$
and type variables $\alpha$. An \emph{abstract refinement type} $\tau$ is 
either a basic type refined with an abstract and concrete refinements,
$\tpref{b}{\areft}{\reft}$, or 
a dependent function type where the parameter $x$ can appear in the 
refinements of the output type. 
We include refinements for functions, as refined type variables can be 
replaced by function types. However, typechecking ensures these refinements
are trivially true.
%
%type application
%Type application consists of a type constructor, its type arguments
%and its refinement arguments 
%that are used to describe properties between its elements.
%
Finally, types can be quantified over refinement variables and type 
variables to yield abstract refinement schemas.


\begin{figure}[t!]
\centering
$$
\begin{array}{rrcl}
\emphbf{Expressions} \quad 
  & e 
  & ::= 
  &      x 
  \spmid c 
  \spmid \efunt{x}{\tau}{e} 
  \spmid \eapp{e}{e} 
  \spmid \etabs{\alpha}{e} 
  \spmid \etapp{e}{\tau} 
  \spmid \epabs{\rvar}{\tau}{e}
  \spmid \epapp{e}{e} 
  \\[0.05in] 

\emphbf{Abstract Refinements} \quad 
  & \areft 
  & ::= 
  &      \true 
  \spmid \areft \land \rvapp{\rvar}{e}
  \\[0.05in] 

\emphbf{Basic Types} \quad 
  & b 
  & ::= 
  &      \tbint
  \spmid \tbbool
  \spmid \alpha
  \\[0.05in]

\emphbf{Abstract Refinement Types} \quad 
  & \tau 
  & ::= 
  &      \tpref{b}{\areft}{\reft} 
  \spmid \trfun{x}{\tau}{\tau}{\reft}
  \\[0.05in]

\emphbf{Abstract Refinement Schemas} \quad 
  & \sigma
  & ::= 
  &      \tau 
  \spmid \ttabs{\alpha}{\sigma}
  \spmid \tpabs{\rvar}{\tau}{\sigma}
  \\[0.05in]
\end{array}
$$
\caption{\textbf{Syntax of Expressions, Refinements, Types and Schemas}}
\label{fig:syntax}
\end{figure}

\subsection{Static Semantics}\label{sec:typing}

\input{rules}

Next, we describe the static semantics of \corelan by describing the typing
judgments and derivation rules. Most of the rules are 
standard~\cite{Ou2004,LiquidPLDI08,Knowles10,GordonTOPLAS2011}; we 
discuss only those pertaining to abstract refinements.

\mypara{Judgments}
A type environment $\Gamma$ is a sequence of type bindings $x:\sigma$.
We use environments to define three kinds of typing judgments:

\begin{itemize}
\item{\emphbf{Wellformedness judgments} (\isWellFormed{\Gamma}{\sigma})} 
state that a type schema $\sigma$ is well-formed under environment
$\Gamma$, that is, the refinements in $\sigma$ are boolean 
expressions in the environment $\Gamma$.

\item{\emphbf{Subtyping judgments} (\isSubType{\Gamma}{\sigma_1}{\sigma_2})} 
state that the type schema $\sigma_1$ is a subtype of the type schema
$\sigma_2$ under environment $\Gamma$, that is, when the free variables
of $\sigma_1$ and $\sigma_2$
are bound to values described by $\Gamma$, the set of values described
by $\sigma_1$ is contained in the set of values described by $\sigma_2$. 

\item{\emphbf{Typing judgments} (\hastype{\Gamma}{e}{\sigma})} state that
the expression $e$ has the type schema $\sigma$ under environment $\Gamma$,
that is, when the free variables in $e$ are bound to values described by 
$\Gamma$, the expression $e$ will evaluate to a value described by $\sigma$.
\end{itemize}

\mypara{Wellformedness Rules}
The wellformedness rules check that the concrete and abstract
refinements are indeed $\tbbool$-valued expressions in the 
appropriate environment.
The key rule is \wtBase, which checks, as usual, that the (concrete) 
refinement $\reft$ is boolean, and additionally, that the abstract
refinement $\areft$ applied to the value $\vref$ is also boolean.
This latter fact is established by \wtRVApp which checks that 
each refinement variable application $\rvapp{\rvar}{e}\ \vref$ 
is also of type \tbbool in the given environment.

\mypara{Subtyping Rules}
The subtyping rules stipulate when the set of values described 
by schema $\sigma_1$ is subsumed by the values described by $\sigma_2$.
The rules are standard except for \tsubVar, which encodes the base types' 
abstract refinements $\areft_1$ and $\areft_2$ with conjunctions of 
\emph{uninterpreted predicates} 
$\inter{\areft_1\ \vref}$ and $\inter{\areft_2\ \vref}$ in the 
refinement logic as follows:
\begin{align*}
\inter{\true\ \vref} & \defeq \true\\
\inter{(\areft \land \rvapp{\rvar}{e})\ \vref} & \defeq \inter{\areft\
\vref} \land \rvar(\inter{e_1},\ldots,\inter{e_n},\vref)
\end{align*}
where $\rvar(\overline{e})$ is a term in the refinement logic corresponding
to the application of the uninterpreted predicate symbol $\rvar$ to the 
arguments $\overline{e}$.
% $\text{Valid}(p)$ (\tsubBase) holds if an SMT determines the formula $p$ 
% is \emph{valid}~\cite{Nelson81}.



\mypara{Type Checking Rules}
The type checking rules are standard except for \tpgen and \tpinst, which
pertain to abstraction and instantiation of abstract refinements.
%
The rule \tpgen is the same as \tfunction: we simply check the body
$e$ in the environment extended with a binding for the refinement 
variable $\rvar$.
%
The rule \tpinst checks that the concrete refinement is of the appropriate
(unrefined) type $\tau$, and then replaces all (abstract) applications of
$\rvar$ inside $\sigma$ with the appropriate (concrete) refinement $\reft'$ 
with the parameters $\overline{x}$ replaced with arguments at that application.
Formally, this is represented as $\rpinst{\sigma}{\rvar}{\efunbar{x:\tau}{\reft'}}$
which is $\sigma$ with each base type transformed as
%%$$\rpinst{\tpref{b}{\areft}{\reft}}{\rvar}{z}
%%  \defeq \tpref{b}{\areft''}{\reft \land \reft''} 
%%  \quad \mbox{where} (\areft'', \reft'') =
%%  \rpapply{\areft}{\rvar}{z}{\true}{\true}$$
\begin{align*}
\rpinst{\tpref{b}{\areft}{\reft}}{\rvar}{z}
  & \defeq \tpref{b}{\areft''}{\reft \land \reft''} \\
\mbox{where} \quad (\areft'', \reft'') 
  & \defeq \rpapply{\areft}{\rvar}{z}{\true}{\true} 
\intertext{$\mathsf{Apply}$ replaces each application of $\rvar$ in 
$\areft$ with the corresponding conjunct in $\reft''$, as}
\rpapply{\true}{\cdot}{\cdot}{\areft'}{\reft'} 
  & \defeq (\areft', \reft') \\
\rpapply{\areft \wedge \rvapp{\rvar'}{e}}{\rvar}{z}{\areft'}{\reft'} 
  & \defeq \rpapply{\areft}{\rvar}{z}{\areft' \land \rvapp{\rvar'}{e}}{\reft'} \\
\rpapply{\areft \wedge \rvapp{\rvar}{e}}{\rvar}{\efunbar{x:\tau}{\reft''}}{\areft'}{\reft'} 
  & \defeq
  \rpapply{\areft}{\rvar}{\efunbar{x:\tau}{\reft''}}{\areft'}{\reft' \wedge \SUBST{\reft''}{\overline{x}}{\overline{e},\vref}}
\end{align*}
In other words, the instantiation can be viewed as two symbolic 
reduction steps: first replacing the refinement variable with the
concrete refinement, and then ``beta-reducing" concrete refinement 
with the refinement variable's arguments. For example, 
$$\rpinst{\tpref{\tbint}{\rvar\ y}{\vref > 10}}
       {\rvar}
       {\efunt{x_1}{\tau_1}{\efunt{x_2}{\tau_2}{x_1 < x_2}}}
\defeq \tref{\tbint}{\vref > 10 \land y < \vref}$$
%%rp(x:tx->t , \rvar, z) = x:tx' -> t'
%%  where tx'      = rp(tx, \rvar, z)
%%        t'       = rp(t , \rvar, z)
%%
%%rp(\a.t, \rvar, z) = \a.t'
%%  where t'       = rp(t, \rvar, z)
%%
%%rp(\p.t, \rvar, z) = \p.t'
%%  where t'       = rp(t, \rvar, z)

%%The other rule that handles abstract refinements is \tcase.
%%This rule initially checks that the expression to be analyzed 
%%has a type application type $T = \tcon{\chi}{e_\chi}{\listOf{T}}{\listOf{e}}$.
%%Then for all cases, the case expression is typechecked in the initial environment, 
%%extended with case binders \listOf{x_i} and the initial expression binder $x$.
%%The types of these binders are gained after unfolding data constructor's type \tc{K_i}. 
%%The unfolding is done by replacing its type variables with actual type arguments
%%of $T$, ie. \listOf{T} 
%%its abstract refinements with actual inferred refinements \listOf{e},
%%and its binders with actual binders \listOf{x_i}.

\subsection{Soundness}\label{sec:soundness}

As hinted by the discussion about refinement variable instantiation,
we can intuitively think of abstract refinement variables as 
\emph{ghost} program variables whose values are boolean-valued 
functions. Hence, abstract refinements are a special case of 
higher-order contracts, that can be statically verified using 
uninterpreted functions. (Since we focus on static checking, 
we don't care about the issue of blame.)
We formalize this notion by translating \corelan programs into
the contract calculus \conlan of \cite{Greenberg11} and use this 
translation to define the dynamic semantics and establish soundness.

\mypara{Translation} 
We translate \corelan schemes $\sigma$ to \conlan schemes $\tx{\sigma}$
as by translating abstract refinements into contracts,
and refinement abstraction into function types:
$$\begin{array}{rclcrcl}
\tx{\true\ \vref} & \defeq 
  & \true  
  & \quad \quad &

\tx{\tpabs{\rvar}{\tau}{\sigma}} & \defeq 
  & \tfun{\rvar}{\tx{\tau}}{\tx{\sigma}} \\

\tx{(\areft \land \rvapp{\rvar}{e})\ \vref} & \defeq 
  & \tx{\areft\ \vref} \land \eapp{\eapp{\rvar}{\overline{e}}}{\vref} 
  & \quad \quad &

\tx{\ttabs{\alpha}{\sigma}} & \defeq 
  & \ttabs{\alpha}{\tx{\sigma}} \\

\tx{\tpref{b}{\areft}{\reft}} & \defeq 
  & \tref{b}{\reft \land \tx{\areft\ \vref}} 
  & \quad \quad &

\tx{\tfun{x}{\tau_1}{\tau_2}} & \defeq 
  & \tfun{x}{\tx{\tau_1}}{\tx{\tau_2}} 
%\tx{\trfun{x}{\tau_1}{\tau_2}{\reft}} \defeq 
%  & \trfun{x}{\tx{\tau_1}}{\tx{\tau_2}}{\tx{\reft}} \\
\end{array}$$
Similarly, we translate \corelan terms $e$ to \conlan 
terms $\tx{e}$ by converting refinement abstraction and application 
to $\lambda$-abstraction and application
$$\begin{array}{rclcrcl}
\tx{x} & \defeq & x & \quad \quad \quad & \tx{c} & \defeq & c \\
\tx{\efunt{x}{\tau}{e}} & \defeq & \efunt{x}{\tx{\tau}}{\tx{e}} & \quad & \tx{\eapp{e_1}{e_2}} & \defeq & \eapp{\tx{e_1}}{\tx{e_2}} \\
\tx{\etabs{\alpha}{e}} & \defeq & \etabs{\alpha}{\tx{e}} & \quad & \tx{\etapp{e}{\tau}} & \defeq & \eapp{\tx{e}}{\tx{\tau}} \\
\tx{\epabs{\rvar}{\tau}{e}} &\defeq & \efunt{\rvar}{\tx{\tau}}{\tx{e}} & \quad & \tx{\epapp{e_1}{e_2}} &\defeq & \eapp{\tx{e_1}}{\tx{e_2}}
\end{array}$$

%%\begin{align*}
%%\tx{\true\ \vref} \defeq 
%%  & \true\\
%%\tx{(\areft \land \rvapp{\rvar}{e})\ \vref} \defeq 
%%  & \tx{\areft\ \vref} \land \eapp{\eapp{\rvar}{\overline{e}}}{\vref}\\
%%\tx{\tpref{b}{\areft}{\reft}} \defeq 
%%  & \tref{b}{\reft \land \tx{\areft\ \vref}} \\
%%\tx{\tfun{x}{\tau_1}{\tau_2}} \defeq 
%%  & \tfun{x}{\tx{\tau_1}}{\tx{\tau_2}} \\
%%%\tx{\trfun{x}{\tau_1}{\tau_2}{\reft}} \defeq 
%%%  & \trfun{x}{\tx{\tau_1}}{\tx{\tau_2}}{\tx{\reft}} \\
%%\tx{\ttabs{\alpha}{\sigma}} \defeq 
%%  & \ttabs{\alpha}{\tx{\sigma}} \\
%%\tx{\tpabs{\rvar}{\tau}{\sigma}} \defeq 
%%  & \tfun{\rvar}{\tx{\tau}}{\tx{\sigma}}
%%\end{align*}
%%\tx{x} \defeq & x \\
%%\tx{c} \defeq & c \\
%%\tx{\efunt{x}{\tau}{e}} \defeq & \efunt{x}{\tx{\tau}}{\tx{e}} \\
%%\tx{\eapp{e_1}{e_2}} \defeq & \eapp{\tx{e_1}}{\tx{e_2}} \\
%%\tx{\etabs{\alpha}{e}} \defeq & \etabs{\alpha}{\tx{e}} \\
%%\tx{\etapp{e}{\tau}} \defeq & \eapp{\tx{e}}{\tx{\tau}} \\
%%\tx{\epabs{\rvar}{\tau}{e}} \defeq & \efunt{\rvar}{\tx{\tau}}{\tx{e}} \\
%%\tx{\epapp{e_1}{e_2}} \defeq & \eapp{\tx{e_1}}{\tx{e_2}}





\mypara{Translation Properties}
We can show by induction on the derivations that the 
type derivation rules of \corelan \emph{conservatively approximate}
those of \conlan. Formally, 

\begin{itemize}
\item If $\isWellFormed{\Gamma}{\tau}$ then $\isWellFormedH{\Gamma}{\tau}$,
\item If $\isSubType{\Gamma}{\tau_1}{\tau_2}$ then $\isSubTypeH{\Gamma}{\tau_1}{\tau_2}$,
\item If $\hastype{\Gamma}{e}{\tau}$ then
$\hastypeH{\tx{\Gamma}}{\tx{e}}{\tx{\tau}}$.
\end{itemize}

\mypara{Soundness} Thus rather than re-prove preservation and progress
for \corelan, we simply use the fact that the type derivations are
conservative to derive the following preservation and progress 
corollaries from \cite{Greenberg11}:
%
\begin{itemize}
\item{\textbf{Preservation: }} 
  If $\hastype{\emptyset}{e}{\tau}$ 
  and $\tx{e} \longrightarrow e'$ 
  then $\hastypeH{\emptyset}{e'}{\tx{\tau}}$

\item{\textbf{Progress: }}
  If $\hastype{\emptyset}{e}{\tau}$, then either
  $\tx{e} \longrightarrow e'$ or 
  $\tx{e}$ is a value.
\end{itemize}
%
Note that, in a contract calculus like \conlan, subsumption is encoded
as a \emph{upcast}. However, if subtyping relation can be statically 
guaranteed (as is done by our conservative SMT based subtyping) 
then the upcast is equivalent to the identity function and can 
be eliminated. Hence, \conlan terms $\tx{e}$ translated from well-typed 
\corelan terms $e$ have no casts.

\subsection{Refinement Inference}\label{sec:infer}

Our design of abstract refinements makes it particularly easy to 
perform type inference via Liquid typing, which is crucial for
making the system usable by eliminating the tedium of instantiating 
refinement parameters all over the code. (With value-dependent 
refinements, one cannot simply use, say, unification to determine
the appropriate instantations, as is done for classical type systems.)
We briefly recall how Liquid types work, and sketch how they are 
extended to infer refinement instantiations.

\mypara{Liquid Types} 
The Liquid Types method infers refinements in three steps. 
%
First, we create refinement \emph{templates} for the unknown, 
to-be-inferred refinement types. The \emph{shape} of the template 
is determined by the underlying (non-refined) type it corresponds to, 
which can be determined from the language's underlying (non-refined) 
type system. 
The template is just the shape refined with fresh refinement variables
$\kappa$ denoting the unknown refinements at each type position. 
For example, from a type ${\tfun{x}{\tbint}{\tbint}}$ we create 
the template ${\tfun{x}{\tref{\tbint}{\kappa_x}}{\tref{\tbint}{\kappa}}}$.
%
Second, we perform type checking using the templates (in place of the
unknown types.) Each wellformedness check becomes a wellformedness
constraint over the templates, and hence over the individual $\kvar$,
constraining which variables can appear in $\kvar$.
Each subsumption check becomes a subtyping constraint
between the templates, which can be further simplified, via syntactic
subtyping rules, to a logical implication query between the variables
$\kappa$.
%
Third, we solve the resulting system of logical implication constraints
(which can be cyclic) via abstract interpretation --- in particular,
monomial predicate abstraction over a set of logical qualifiers
\cite{Houdini,LiquidPLDI08}. The solution is a map from $\kvar$ to
conjunctions of qualifiers, which, when plugged back into the templates,
yields the inferred refinement types.

\mypara{Inferring Refinement Instantiations}
The key to making abstract refinements practical is a means of 
synthesizing the appropriate arguments $\reft'$ for each refinement 
application $\epapp{e}{\reft'}$. 
Note that for such applications, we can, from $e$, determine the 
non-refined type of $\reft'$, which is of the form 
${\tau_1 \rightarrow \ldots \rightarrow \tau_n \rightarrow \tbbool}$.
Thus, $\reft'$ has the template 
${\efunt{x_1}{\tau_1}{\ldots \efunt{x_n}{\tau_n}{\kvar}}}$
where $\kvar$ is a fresh, unknown refinement variable that 
must be solved to a boolean valued expression over $x_1,\ldots,x_n$.
Thus, we generate a \emph{wellformedness} constraint 
${\isWellFormed{x_1:\tau_1, \ldots, x_n:\tau_n}{\kvar}}$
and carry out typechecking with template, which, as before, yields
implication constraints over $\kvar$, which can, as before, be 
solved via predicate abstraction.
Finally, in each refinement template, we replace each $\kvar$ with its
solution $e_\kvar$ to get the inferred refinement instantiations.

%%To infer appropabstract refinements we used the liquid type variables
%%$\kappa$ with explicit arguments to avoid inferring function 
%%expressions:
%%To infer an expression to replace a predicate of type 
%%$\listOf{x_i:\tau_i; \tau}$ in an environment $\Gamma$, 
%%we create a fresh liquid variable $\kappa$ on $\tau$ which is
%%wellformed in the environment $\Gamma$ extended with the bindings
%%\listOf{x_i:\tau_i}.
%%When $\kvar$ is solved via predicate abstraction to an expression 
%%$e_\kvar$, we simply replace $\kvar$ with 
%%the set as the inferred expression 
%%$e =\efun{x_1}{\dots\efun{x_n}{\efun{v}{e_\kappa}}}$.
%add a refinement variable in place of expressions. 
%\mypara{Constants}\jhala{constant-refinements and soundness guarantees?}
%%TODO: 
%%[SKIP] add paragraph on constants to opsem
%%[SKIP] redefine \reft to r? (to emphasize not arbitrary expression?)


